ASlib: A Benchmark Library for Algorithm Selection

The task of algorithm selection involves choosing an algorithm from a set of algorithms on a per-instance basis in order to exploit the varying performance of algorithms over a set of instances. The algorithm selection problem is attracting increasing attention from researchers and practitioners in AI. Years of fruitful applications in a number of domains have resulted in a large amount of data, but the community lacks a standard format or repository for this data. This situation makes it difficult to share and compare different approaches effectively, as is done in other, more established fields. It also unnecessarily hinders new researchers who want to work in this area. To address this problem, we introduce a standardized format for representing algorithm selection scenarios and a repository that contains a growing number of data sets from the literature. Our format has been designed to be able to express a wide variety of different scenarios. Demonstrating the breadth and power of our platform, we describe a set of example experiments that build and evaluate algorithm selection models through a common interface. The results display the potential of algorithm selection to achieve significant performance improvements across a broad range of problems and algorithms.

==> pics/as_tikz_complex.tex <==
\tikzstyle{activity}=[rectangle, draw=black, rounded corners, text centered, text width=9em, fill=white, drop shadow]
\tikzstyle{data}=[rectangle, draw=black, text centered, fill=black!10, text width=9em, drop shadow]
\tikzstyle{myarrow}=[->, thick]
\begin{tikzpicture}[align=center,node distance=3.7cm]
	
	\node (perf) [data] {Performance Data: $\mathcal{I} \times \mathcal{A} \to \mathbb{R}$};
	\node (feat) [data, below of=perf, yshift=2.3cm] {Feature Data: $f: \mathcal{I} \to \mathcal{F}$};
	\node (cost) [data, below of=feat, yshift=2.3cm] {Feature Costs: $c: \mathcal{P}(\mathcal{I}) \to \mathbb{R}$};
	
	\node (train) [activity, right of=feat, text width=10em] {Train\\ $\mathcal{F} \to (\phi: \mathbb{N} \to \mathcal{A} \times \mathbb{R}_{0}^+)$};
	
	\node (run) [activity, right of=train, xshift=0.5cm] {Select\\ $a_1, t_1 = \phi_{f(i)}(1)$ and apply $a_1$ for time $t_1$ to $i$};
	\node (run2) [activity, right of=run, xshift=0.5cm] {Select\\ $a_2, t_2 = \phi_{f(i)}(2)$ and apply $a_2$ for time $t_2$ to $i$};
	
	\node (feat_i) [activity, above of=run, yshift=-2.0cm] {Compute Features $f(i)$ of $i$};
	\node (inst) [data, above of=feat_i, yshift=-2.3cm] {(New) Instance $i$};
	
	\node (eva) [activity, below of=run, yshift=1.5cm] {Evaluate $m(i, \phi_{f(i)}(1))$ and $c(f(i))$};
	\node (eva2) [activity, below of=run2, yshift=1.5cm, text width=11em] {Evaluate $\sum_{j=1}^{2}m(i, \phi_{f(i)}(j))$ and $c(f(i))$};
	
	\draw[myarrow] (perf) -| (train.north);
	\draw[myarrow] (feat) -- (train.west);
	\draw[myarrow] (cost) -| (train.south);
	
	\draw[myarrow] (inst) -- (feat_i);
	\draw[myarrow] (feat_i) -- (run);
	\draw[myarrow] (train) -- (run);
	\draw[myarrow] (run) -- node [left] {success} (eva);
	\draw[myarrow] (run) -- node [above] {fail}  (run2);
	\draw[myarrow] (run2) -- node [left] {success} (eva2);
	\draw[myarrow] (run2) -- node [above] {fail} ($(run2.east)+(1.0,0)$);
	
	\path (train.east -| train.east)+(0.4,4.2) node (a) {};
    \path (train.east |- train.east)+(0.4,-3.5) node(b) {};
    \draw[dashed, color=black!60] (a) -- (b);
    \path[color=black!60] (train.east -| train.east)+(-0.3,3.8) node (a) {Offline};
    \path[color=black!60] (train.east -| train.east)+(1.0,3.8) node (a) {Online};
	
\end{tikzpicture}

==> results.tex <==
\begin{table}[ht]
\subfloat[caption][ASP-POTASSCO]{
\footnotesize{
% latex table generated in R 3.1.0 by xtable 1.7-4 package
% Tue Jan 27 11:27:36 2015
\begin{tabular}{llrrr}
  \toprule
Type & Model & Solved & PAR10 & MCP \\ 
  \midrule
baseline & singleBestByPar & 0.86 & 880.5 & 58.9 \\ 
  baseline & singleBestByPar & 0.86 & 880.5 & 58.9 \\ 
  baseline & vbs & 0.94 & 400.2 & 0.0 \\ 
  baseline & vbs & 0.94 & 400.2 & 0.0 \\ 
  classif & ksvm & 0.89 & 692.0 & 32.0 \\ 
  classif & randomForest & 0.88 & 712.2 & 31.4 \\ 
  classif & rpart & 0.89 & 655.0 & 28.4 \\ 
  cluster & XMeans & 0.89 & 701.8 & 37.7 \\ 
  regr & lm & 0.90 & 615.1 & 26.1 \\ 
  regr & randomForest & 0.92 & 509.1 & 16.0 \\ 
  regr & rpart & 0.90 & 624.9 & 31.7 \\ 
   \bottomrule
\end{tabular}
}
}
\subfloat[caption][CSP-2010]{
\footnotesize{
% latex table generated in R 3.1.0 by xtable 1.7-4 package
% Tue Jan 27 11:27:36 2015
\begin{tabular}{rrr}
  \toprule
Solved & PAR10 & MCP \\ 
  \midrule
0.86 & 7201.6 & 79.1 \\ 
  0.86 & 7201.6 & 79.1 \\ 
  0.88 & 6344.3 & 0.0 \\ 
  0.88 & 6344.3 & 0.0 \\ 
  0.87 & 6558.8 & 14.4 \\ 
  0.87 & 6677.6 & 22.1 \\ 
  0.87 & 6488.2 & 10.5 \\ 
  0.86 & 7005.4 & 60.8 \\ 
  0.87 & 6633.5 & 22.4 \\ 
  0.87 & 6466.7 & 11.3 \\ 
  0.86 & 6928.0 & 50.1 \\ 
   \bottomrule
\end{tabular}
}
}
\end{table}
\begin{table}[ht]
\subfloat[caption][MAXSAT12-PMS]{
\footnotesize{
% latex table generated in R 3.1.0 by xtable 1.7-4 package
% Tue Jan 27 11:27:36 2015
\begin{tabular}{llrrr}
  \toprule
Type & Model & Solved & PAR10 & MCP \\ 
  \midrule
baseline & singleBestByPar & 0.77 & 4893.1 & 190.9 \\ 
  baseline & singleBestByPar & 0.77 & 4893.1 & 190.9 \\ 
  baseline & vbs & 0.85 & 3127.2 & 0.0 \\ 
  baseline & vbs & 0.85 & 3127.2 & 0.0 \\ 
  classif & ksvm & 0.83 & 3553.7 & 38.0 \\ 
  classif & randomForest & 0.82 & 3744.8 & 56.5 \\ 
  classif & rpart & 0.82 & 3795.5 & 64.1 \\ 
  cluster & XMeans & 0.82 & 3833.9 & 80.9 \\ 
  regr & lm & 0.82 & 3777.9 & 68.0 \\ 
  regr & randomForest & 0.84 & 3367.6 & 24.5 \\ 
  regr & rpart & 0.82 & 3789.7 & 79.8 \\ 
   \bottomrule
\end{tabular}
}
}
\subfloat[caption][PREMARSHALLING-ASTAR-2013]{
\footnotesize{
% latex table generated in R 3.1.0 by xtable 1.7-4 package
% Tue Jan 27 11:27:36 2015
\begin{tabular}{rrr}
  \toprule
Solved & PAR10 & MCP \\ 
  \midrule
0.81 & 7002.9 & 688.8 \\ 
  0.81 & 7002.9 & 688.8 \\ 
  1.00 & 227.6 & 0.0 \\ 
  1.00 & 227.6 & 0.0 \\ 
  0.86 & 5172.5 & 518.3 \\ 
  0.85 & 5688.9 & 542.9 \\ 
  0.88 & 4634.2 & 471.9 \\ 
  0.85 & 5756.4 & 548.9 \\ 
  0.84 & 5885.1 & 554.6 \\ 
  0.85 & 5546.5 & 523.5 \\ 
  0.85 & 5645.9 & 561.4 \\ 
   \bottomrule
\end{tabular}
}
}
\end{table}
\begin{table}[ht]
\subfloat[caption][PROTEUS-2014]{
\footnotesize{
% latex table generated in R 3.1.0 by xtable 1.7-4 package
% Tue Jan 27 11:27:36 2015
\begin{tabular}{llrrr}
  \toprule
Type & Model & Solved & PAR10 & MCP \\ 
  \midrule
baseline & singleBestByPar & 0.63 & 13443.3 & 957.5 \\ 
  baseline & singleBestByPar & 0.63 & 13443.3 & 957.5 \\ 
  baseline & vbs & 0.89 & 4105.9 & 0.0 \\ 
  baseline & vbs & 0.89 & 4105.9 & 0.0 \\ 
  classif & ksvm & 0.81 & 6863.7 & 288.5 \\ 
  classif & randomForest & 0.81 & 6873.8 & 288.6 \\ 
  classif & rpart & 0.77 & 8527.0 & 451.9 \\ 
  cluster & XMeans & 0.78 & 8171.2 & 436.3 \\ 
  regr & lm & 0.78 & 7975.6 & 403.6 \\ 
  regr & randomForest & 0.84 & 6066.6 & 211.9 \\ 
  regr & rpart & 0.81 & 6921.3 & 302.2 \\ 
   \bottomrule
\end{tabular}
}
}
\subfloat[caption][QBF-2011]{
\footnotesize{
% latex table generated in R 3.1.0 by xtable 1.7-4 package
% Tue Jan 27 11:27:36 2015
\begin{tabular}{rrr}
  \toprule
Solved & PAR10 & MCP \\ 
  \midrule
0.58 & 15330.2 & 716.8 \\ 
  0.58 & 15330.2 & 716.8 \\ 
  0.77 & 8337.1 & 0.0 \\ 
  0.77 & 8337.1 & 0.0 \\ 
  0.71 & 10428.7 & 220.5 \\ 
  0.73 & 9776.1 & 160.1 \\ 
  0.72 & 10316.9 & 227.2 \\ 
  0.67 & 12089.1 & 412.5 \\ 
  0.71 & 10388.7 & 227.9 \\ 
  0.75 & 9075.0 & 98.4 \\ 
  0.71 & 10405.5 & 244.7 \\ 
   \bottomrule
\end{tabular}
}
}
\end{table}
\begin{table}[ht]
\subfloat[caption][SAT11-HAND]{
\footnotesize{
% latex table generated in R 3.1.0 by xtable 1.7-4 package
% Tue Jan 27 11:27:36 2015
\begin{tabular}{llrrr}
  \toprule
Type & Model & Solved & PAR10 & MCP \\ 
  \midrule
baseline & singleBestByPar & 0.50 & 25589.3 & 1434.7 \\ 
  baseline & singleBestByPar & 0.50 & 25589.3 & 1434.7 \\ 
  baseline & vbs & 0.74 & 13360.7 & 0.0 \\ 
  baseline & vbs & 0.74 & 13360.7 & 0.0 \\ 
  classif & ksvm & 0.66 & 17446.9 & 406.1 \\ 
  classif & randomForest & 0.66 & 17655.5 & 462.7 \\ 
  classif & rpart & 0.62 & 19126.8 & 567.1 \\ 
  cluster & XMeans & 0.50 & 25272.9 & 1094.8 \\ 
  regr & lm & 0.60 & 20251.4 & 629.7 \\ 
  regr & randomForest & 0.67 & 16906.5 & 321.9 \\ 
  regr & rpart & 0.61 & 19929.2 & 611.0 \\ 
   \bottomrule
\end{tabular}
}
}
\subfloat[caption][SAT11-INDU]{
\footnotesize{
% latex table generated in R 3.1.0 by xtable 1.7-4 package
% Tue Jan 27 11:27:36 2015
\begin{tabular}{rrr}
  \toprule
Solved & PAR10 & MCP \\ 
  \midrule
0.72 & 14605.9 & 718.4 \\ 
  0.72 & 14605.9 & 718.4 \\ 
  0.84 & 8187.5 & 0.0 \\ 
  0.84 & 8187.5 & 0.0 \\ 
  0.73 & 14004.7 & 602.9 \\ 
  0.74 & 13655.1 & 541.5 \\ 
  0.72 & 14336.4 & 622.8 \\ 
  0.68 & 16299.2 & 810.8 \\ 
  0.72 & 14460.5 & 611.9 \\ 
  0.75 & 12996.6 & 494.3 \\ 
  0.69 & 15884.7 & 684.4 \\ 
   \bottomrule
\end{tabular}
}
}
\end{table}
\begin{table}[ht]
\subfloat[caption][SAT11-RAND]{
\footnotesize{
% latex table generated in R 3.1.0 by xtable 1.7-4 package
% Tue Jan 27 11:27:36 2015
\begin{tabular}{llrrr}
  \toprule
Type & Model & Solved & PAR10 & MCP \\ 
  \midrule
baseline & singleBestByPar & 0.60 & 19916.4 & 979.9 \\ 
  baseline & singleBestByPar & 0.60 & 19916.4 & 979.9 \\ 
  baseline & vbs & 0.82 & 9186.4 & 0.0 \\ 
  baseline & vbs & 0.82 & 9186.4 & 0.0 \\ 
  classif & ksvm & 0.78 & 11164.6 & 156.0 \\ 
  classif & randomForest & 0.79 & 10838.3 & 129.8 \\ 
  classif & rpart & 0.79 & 10602.7 & 118.6 \\ 
  cluster & XMeans & 0.78 & 11337.7 & 178.9 \\ 
  regr & lm & 0.78 & 11275.4 & 191.5 \\ 
  regr & randomForest & 0.80 & 10341.2 & 82.2 \\ 
  regr & rpart & 0.76 & 12017.1 & 259.1 \\ 
   \bottomrule
\end{tabular}
}
}
\subfloat[caption][SAT12-ALL]{
\footnotesize{
% latex table generated in R 3.1.0 by xtable 1.7-4 package
% Tue Jan 27 11:27:36 2015
\begin{tabular}{rrr}
  \toprule
Solved & PAR10 & MCP \\ 
  \midrule
0.75 & 3079.9 & 302.5 \\ 
  0.75 & 3079.9 & 302.5 \\ 
  0.99 & 241.3 & 0.0 \\ 
  0.99 & 241.3 & 0.0 \\ 
  0.91 & 1195.7 & 95.4 \\ 
  0.93 & 1017.2 & 70.4 \\ 
  0.79 & 2643.6 & 219.3 \\ 
  0.74 & 3188.9 & 294.2 \\ 
  0.88 & 1517.5 & 128.8 \\ 
  0.93 & 980.3 & 65.6 \\ 
  0.83 & 2109.3 & 176.9 \\ 
   \bottomrule
\end{tabular}
}
}
\end{table}
\begin{table}[ht]
\subfloat[caption][SAT12-HAND]{
\footnotesize{
% latex table generated in R 3.1.0 by xtable 1.7-4 package
% Tue Jan 27 11:27:36 2015
\begin{tabular}{llrrr}
  \toprule
Type & Model & Solved & PAR10 & MCP \\ 
  \midrule
baseline & singleBestByPar & 0.48 & 6338.9 & 254.8 \\ 
  baseline & singleBestByPar & 0.48 & 6338.9 & 254.8 \\ 
  baseline & vbs & 0.70 & 3662.2 & 0.0 \\ 
  baseline & vbs & 0.70 & 3662.2 & 0.0 \\ 
  classif & ksvm & 0.63 & 4552.5 & 85.9 \\ 
  classif & randomForest & 0.63 & 4511.4 & 72.9 \\ 
  classif & rpart & 0.56 & 5408.5 & 154.8 \\ 
  cluster & XMeans & 0.49 & 6149.3 & 221.0 \\ 
  regr & lm & 0.62 & 4626.4 & 89.3 \\ 
  regr & randomForest & 0.65 & 4252.9 & 53.1 \\ 
  regr & rpart & 0.56 & 5360.0 & 148.4 \\ 
   \bottomrule
\end{tabular}
}
}
\subfloat[caption][SAT12-INDU]{
\footnotesize{
% latex table generated in R 3.1.0 by xtable 1.7-4 package
% Tue Jan 27 11:27:36 2015
\begin{tabular}{rrr}
  \toprule
Solved & PAR10 & MCP \\ 
  \midrule
0.73 & 3332.1 & 148.2 \\ 
  0.73 & 3332.1 & 148.2 \\ 
  0.82 & 2221.5 & 0.0 \\ 
  0.82 & 2221.5 & 0.0 \\ 
  0.76 & 3066.0 & 71.4 \\ 
  0.77 & 2853.6 & 44.3 \\ 
  0.70 & 3677.7 & 127.9 \\ 
  0.71 & 3607.1 & 128.0 \\ 
  0.76 & 3013.8 & 74.6 \\ 
  0.77 & 2837.4 & 45.4 \\ 
  0.73 & 3399.1 & 113.1 \\ 
   \bottomrule
\end{tabular}
}
}
\end{table}
\begin{table}[ht]
\subfloat[caption][SAT12-RAND]{
\footnotesize{
% latex table generated in R 3.1.0 by xtable 1.7-4 package
% Tue Jan 27 11:27:36 2015
\begin{tabular}{llrrr}
  \toprule
Type & Model & Solved & PAR10 & MCP \\ 
  \midrule
baseline & singleBestByPar & 0.73 & 3271.1 & 49.4 \\ 
  baseline & singleBestByPar & 0.73 & 3271.1 & 49.4 \\ 
  baseline & vbs & 0.76 & 2872.8 & 0.0 \\ 
  baseline & vbs & 0.76 & 2872.8 & 0.0 \\ 
  classif & ksvm & 0.73 & 3245.4 & 42.5 \\ 
  classif & randomForest & 0.73 & 3300.3 & 50.0 \\ 
  classif & rpart & 0.74 & 3176.5 & 36.9 \\ 
  cluster & XMeans & 0.74 & 3149.6 & 33.7 \\ 
  regr & lm & 0.73 & 3254.6 & 43.7 \\ 
  regr & randomForest & 0.74 & 3210.3 & 39.1 \\ 
  regr & rpart & 0.72 & 3382.5 & 60.8 \\ 
   \bottomrule
\end{tabular}
}
}
\end{table}


==> results_top_tables.tex <==
\begin{table}[htb]
\begin{center}
\scriptsize
\begin{tabular}{lccc}
\toprule
 & 1st & 2nd & 3rd\\
\midrule
\pbox{.25\textwidth}{SAT11-HAND} & classif/ksvm & regr/randomForest & classif/randomForest\\
 & 0.656 & 0.688 & 0.702\\[.5em]
\pbox{.25\textwidth}{SAT11-INDU} & classif/randomForest & regr/lm & classif/rpart\\
 & 0.935 & 0.942 & 0.953\\[.5em]
\pbox{.25\textwidth}{SAT11-RAND} & regr/randomForest & classif/rpart & classif/randomForest\\
 & 0.515 & 0.534 & 0.544\\[.5em]
\pbox{.25\textwidth}{SAT12-ALL} & regr/randomForest & classif/randomForest & classif/ksvm\\
 & 0.339 & 0.352 & 0.418\\[.5em]
\pbox{.25\textwidth}{SAT12-HAND} & regr/randomForest & classif/randomForest & classif/ksvm\\
 & 0.682 & 0.704 & 0.747\\[.5em]
\pbox{.25\textwidth}{SAT12-INDU} & regr/randomForest & classif/randomForest & classif/ksvm\\
 & 0.848 & 0.859 & 0.88\\[.5em]
\pbox{.25\textwidth}{SAT12-RAND} & classif/rpart & regr/lm & regr/randomForest\\
 & 0.958 & 0.966 & 0.969\\[.5em]
\pbox{.25\textwidth}{SAT15-INDU} & regr/randomForest & classif/ksvm & classif/randomForest\\
 & 0.725 & 0.859 & 0.879\\[.5em]
\pbox{.25\textwidth}{QBF-2011} & regr/randomForest & classif/randomForest & classif/rpart\\
 & 0.599 & 0.641 & 0.671\\[.5em]
\pbox{.25\textwidth}{QBF-2014} & regr/randomForest & classif/randomForest & regr/rpart\\
 & 0.619 & 0.744 & 0.749\\[.5em]
\pbox{.25\textwidth}{MAXSAT12-PMS} & regr/randomForest & classif/randomForest & regr/lm\\
 & 0.674 & 0.765 & 0.772\\[.5em]
\pbox{.25\textwidth}{MAXSAT15-PMS-INDU} & regr/randomForest & regr/lm & cluster/XMeans\\
 & 0.748 & 0.82 & 0.824\\[.5em]
\pbox{.25\textwidth}{CSP-2010} & classif/rpart & regr/randomForest & classif/randomForest\\
 & 0.901 & 0.908 & 0.921\\[.5em]
\pbox{.25\textwidth}{CSP-MZN-2013} & regr/randomForest & regr/lm & classif/ksvm\\
 & 0.478 & 0.523 & 0.531\\[.5em]
\pbox{.25\textwidth}{PROTEUS-2014} & regr/randomForest & regr/lm & classif/randomForest\\
 & 0.436 & 0.465 & 0.492\\[.5em]
\pbox{.25\textwidth}{ASP-POTASSCO} & regr/randomForest & regr/lm & regr/rpart\\
 & 0.562 & 0.698 & 0.71\\[.5em]
\pbox{.25\textwidth}{PREMAR-ASTAR-2015} & \\
 & \\[.5em]
\bottomrule
\end{tabular}
\caption{Best performing approaches (by PAR10) across all data sets. The number underneath the name of the approach is the factor compared to the single best and has been rounded to three digits. That is, 0.5 means that the respective approach had a PAR10 score that was 0.5 times the score of the single best.}
\label{tab:top}
\end{center}
\end{table}

